Communication-reduced Conjugate Gradient Variants for GPU-accelerated Clusters

Linear solvers are key components in any software platform for scientific and engineering computing. The solution of large and sparse linear systems lies at the core of physics-driven numerical simulations relying on partial differential equations (PDEs) and often represents a significant bottleneck in datadriven procedures, such as scientific machine learning. In this paper, we present an efficient implementation of the preconditioned s-step Conjugate Gradient (CG) method, originally proposed by Chronopoulos and Gear in 1989, for large clusters of Nvidia GPU-accelerated computing nodes. The method, often referred to as communication-reduced or communication-avoiding CG, reduces global synchronizations and data communication steps compared to the standard approach, enhancing strong and weak scalability on parallel computers. Our main contribution is the design of a parallel solver that fully exploits the aggregation of low-granularity operations inherent to the s-step CG method to leverage the high throughput of GPU accelerators. Additionally, it applies overlap between data communication and computation in the multi-GPU sparse matrix-vector product. Experiments on classic benchmark datasets, derived from the discretization of the Poisson PDE, demonstrate the potential of the method.

==> algoritmonuovo.tex <==
%
\begin{algorithm}
  \caption{PCGs(A, b, B, x0, s, rtol, kmax) (Part 1)}
  \label{alg:pcgs}
  \begin{algorithmic}[1]
  \State $x=x_0 \ \ r=b-A x_0$
    \For{$k=0,1,...,kmax$}
    \If{($k== 0$)}
       \State $pMPK(A,r,s,B)$
        \State $Q2 = Z$
        \State $UR2 = P(:,2:end)$
        \State $W = Q2^T \cdot UR2$
        \State $b1 = Q2^T \cdot P(:,1)$
	\State Solve for $\alpha$: $W \alpha = b1$
        \State $x = x+Q2 \cdot \alpha$        
        \State $r = r-UR2 \cdot \alpha$        
        \State $pMPK(A,r,s,B)$
        \State $Q1 = Z$
        \State $UR1 = P(:,2:end)$
    \ElsIf{ ($K>0 \&\& k \bmod 2 == 1$)}
       \State $SW(s,W,Z,P,\alpha)$
        \State $Q1 = Q1 + Q2 \cdot \beta$ 
        \State $UR1 = UR1 + UR2 \cdot \beta$

         \State $x = x + Q1 \cdot \alpha$
        \State $r= r -UR1 \cdot \alpha$
        
        \State $pMPK(A,r,s,B)$  
        \State $Q2 = Z$
        \State $UR2 = P(:,2:end)$
    \algstore{bkbreak}
\end{algorithmic}
\end{algorithm}

     \addtocounter{algorithm}{-1}
\begin{algorithm}
  \caption{PCGs(A, b, B, x0, s, rtol, kmax) (Part 2)}
  \begin{algorithmic}[1]
  \algrestore{bkbreak}
  \ElsIf{($k\bmod 2 == 1$)}
    \State $SW(s,W,Z,P,alpha)$
       \State $Q2 = Q2 + Q1 \cdot \beta$
        \State  $UR2 = UR2 + UR1 \cdot \beta$
        
        \State $x= x + Q2 \cdot  \alpha$
        \State $r = r -UR2 \cdot \alpha$

        \State $pMPK(A,r,s,prec)$
        \State $Q1 = Z$
        \State $UR1 = P(:,2:end)$
    \EndIf
    \If{($\|r\| < rtol$)}
        \State return $x$
    \EndIf
    \EndFor
    \State Return error, algorithm did not converge within $kmax$ iterations
  \end{algorithmic}
\end{algorithm}
%
\begin{algorithm}
  \caption{Preconditioned MP Kernel $pMPK(A,r,s,B)$}
  \label{alg:pMPcg}
  \begin{algorithmic}[1]
  \For{$i=1,...,s$}
           \If{$i == 1$}
                \State $P(:, i) = r$
                \State $Z(:, i) = B^{-1} \cdot P(:, i)$
            \Else
               \State $ P(:, i) = A Z(:, i-1)$
               \State $Z(:, i) = B^{-1} \cdot P(:, i)$
           \EndIf
    \EndFor
    \State $P(:,s+1)=A \cdot Z(:,s)$
    \State return $Z, P$
  \end{algorithmic}
\end{algorithm}
%
\begin{algorithm}
  \caption{Scalar Work $SW(s, W, Z, P, \alpha)$}
  \label{alg:pSWcg}
  \begin{algorithmic}[1]
        \State $Wnew = Z^T \cdot P(:,2:end)$
        \State $b2=Z' \cdot P(:,1)$
        \State $rhs=zeros(2s-1,1)$
        \For{$i=1:s$}
	\State $rhs(s-1+i)=b2(i)$
    	\For{$j=1:i-1$}
    	\State $rhs(s-1+i)=rhs(s-1+i)+rhs(s-1+j)\alpha(s-i+j)$
    	\EndFor
    	\State $rhs(s-1+i)= -rhs(s-1+i)/\alpha(s)$
    	\EndFor
 	\For{$i=1:s$}
    	\For{$j=1:i-1$}
    	\State $b1(i,j)= -rhs(i+j-1)$
    	\EndFor
    	\EndFor
	\State Solve for $\beta$: $W\beta = b1$
	\State $W=Wnew-b1 \cdot \beta$  	
	\State Solve for $\alpha$: $W\alpha = b2$
    \State return $\alpha,\beta,W$
  \end{algorithmic}
\end{algorithm}
%
Algorithm \ref{alg:pcgs}, at each iteration, requires the application of the so-called preconditioned Matrix-Power (MP) kernel described in Algorithm \ref{alg:pMPcg}, where a preconditioner application and an SpMV operation are applied alternately, for a total of $s$ preconditioner applications and $s$ SpMV. Furthermore, Algorithms \ref{alg:pcgs} and  \ref{alg:pSWcg}  compute the reduced matrix $W$ and the right-hand side terms by $2s$ dot products simultaneously. Algorithm \ref{alg:pSWcg} executes $\sum_{i=1}^s i=\mathcal{O}(s^2/2)$ floating-point operations to update a vector and two linear system solution of dimension $s$. These last operations represent a computational overhead, which can be locally performed in a parallel setting and is generally amortized by the $\mathcal{O}(s)$ reduction in global synchronization steps with respect to the classic PCG formulation as in Algorithm \ref{alg:pcghs1}. Finally, 
$s$ axpy operations (some of them written in terms of $s$-dimensional matrix rows update) are computed.
